On Distribution Grid Optimal Power Flow Development and Integration

Due to changes in electric distribution grid operation, new operation regimes have been recommended. Distribution grid optimal power flow (DOPF) has received tremendous attention in the research community, yet it has not been fully adopted across the utility industry. Our paper recognizes this problem and suggests a development and integration procedure for DOPF. We propose development of DOPF as a three step procedure of 1) processing the grid, 2) obtaining a tractable solution, and 3) implementing multiple solution algorithms and benchmarking them to improve application reliability. For the integration of DOPF, we demonstrate how a DOPF federate may be developed that can be integrated in a co-simulation environment to mimic the real-world conditions and hence improve its practicality to be deployed in the field. To demonstrate the efficacy of the proposed methods, tests on IEEE 123-bus system are performed where the usage of tractable formulation in DOPF algorithm development and its comparison to the benchmark solution are demonstrated.

==> case_studies_old.tex <==
\section{Case Studies and Analysis}\label{Sec:Results}
This section presents results from the implemented DOPF core features. 
\subsection{Linear Model Analysis}

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figs/flow_plot_node12.png}
\caption{Line flow linearization results of three phases of one of the 13 Node circuit lines.}
 \label{fig-flow-linearizations}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figs/Flow_val_123.eps}
\caption{Line flow linearization results of 123 Bus System.}
 \label{fig-flow-linearizations_123I}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figs/v_plot_node0.png}
\caption{Node voltage linearization results for three phases of one of the 13 Node circuit node.}
 \label{fig-flow-linearizations}
\end{figure}


\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figs/Volt_val_123.eps}
\caption{Node voltage linearization results for 123 Bus System.}
 \label{fig-flow-linearizations_123V}
\end{figure}


\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figs/losses_plot.png}
\caption{Total active and reactive power loss linearization results.}
 \label{fig-flow-linearizations}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figs/Loss_val_123.eps}
\caption{Total active and reactive power loss linearization results for 123 bus.}
 \label{fig-flow-linearizations_123L}
\end{figure}

\subsection{Solution Benchmark}
\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figs/solution_plot.png}
\caption{Bench-marking distributed solution across iterations (solid lines) with the central LP/QP solution (dotted line) obtained from an off-the-shelf solver.}
 \label{fig-flow-linearizations}
\end{figure}


\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figs/C_v_D_123.eps}
\caption{Bench-marking distributed solution across iterations (solid lines) with the central LP/QP solution (dotted line) obtained from an off-the-shelf solver for 123 Bus.}
 \label{ooo}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figs/C_v_D_123_Q.eps}
\caption{Bench-marking distributed solution across iterations (solid lines) with the central LP/QP solution (dotted line) obtained from an off-the-shelf solver for 123 Bus.}
 \label{ooo}
\end{figure}


\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figs/statistics_plot.png}
\caption{Statistics of 100 randomly initialized flexibility constraints and primal variable initial values.}
 \label{fig-flow-linearizations}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figs/C_v_D_123_Stat.eps}
\caption{Statistics of 100 randomly initialized flexibility constraints and primal variable initial values for 123 bus.}
 \label{fig-flow-linearizations}
\end{figure}
% The proposed algorithm is demonstrated on a real world distribution system located off the coast of Massachusetts\cite{Nantucket.2019}. The grid contains 12,796 nodes with single and three phase transmission lines, capacitor banks and voltage regulators, to serve the peak load of 51 MW.  

% From the grid side, two inequalities: i) maximum line current and ii) minimum and maximum voltage limits: and one equality constraint iii) active power losses, are considered. From the technology optimization only inequality constraints of maximum and minimum values of the setpoints are considered. This means that the feasibility check from the technology module only consists of projecting the modified setpoints to its allowable maximum/minimum range. Moreover, as the focus is towards coordinating modules through the proposed OPF, the inter-temporal technology module constraints are omitted.

% The line currents at one of the major lines in the feeder is selected as a hard constraint, whereas the grid voltages are taken as soft constraints. This is because all voltages of a heavily loaded grid to be in between minimum/maximum limits of 0.95/1.05 is not realistic, as it requires very large-scale dispersed flexible technologies deployment. The algorithm was implemented using MATLAB whereas the grid module is implemented using OpenDSS \cite{openDSS.2018}. 
% \vspace{-0.1cm}
% \subsection{Controllable Loads Optimization}
% \vspace{-0.1cm}
% For this scenario, 21 controllable loads are assumed as the technology to be optimized, uniformly dispersed across the network with minimum/maximum power of 0/60 kW and sensitivity factor to represent cost of deviating from the preferred schedule as 2 units/$\text{MW}^{2}$ (see cost model in \cref{sensitivityderivations}). 
% \begin{figure}[h]
% \centering
% \includegraphics[width=0.5\textwidth,height=0.4\textwidth]{extras/Figures/controllable_loads.eps}
% \caption{The optimized controllable loads (top), line currents of the line used as hard constraints (middle) and the grid losses (bottom).}
%  \label{fig-controllableloads}
% \end{figure}
% \Cref{fig-controllableloads} demonstrates how coordinating optimal power flow attempts to adhere to the grid constraints, while satisfying the controllable loads feasibility. Some oscillations observed around iterations 10, 15 and 43 are because of legacy control changes (capacitors/regulators) to provide internal voltage support by the grid module. The proposed method brings line currents to their allowable limits by reducing controllable loads, which consequently also decrease losses. The algorithm terminates in 43 iterations and the overall optimization takes less than 3 minutes.
% \begin{figure}[h]
% \centering
% \includegraphics[width=0.45\textwidth,width=0.35\textwidth]{extras/Figures/voltages.eps}
% \caption{Voltage magnitude before and after the proposed  coordinating OPF.}
%  \label{fig-voltages}
% \end{figure}
% \Cref{fig-voltages} compares the original grid voltages to the ones obtained from the proposed algorithm. The proposed method yields an improved overall voltage profile, by yielding 143 lesser minimum voltage violation counts as compared to the original voltages.
% \begin{figure}[h]
% \centering
% \includegraphics[width=0.35\textwidth, height=0.25\textwidth]{extras/Figures/RealPower.png}
% \caption{Assumed real power profile for BESS.}
%  \label{fig-RealPower}
% \end{figure}
% \vspace{-0.15cm}
% \subsection{Battery Energy Storage System (BESS) Optimization}\vspace{-0.1cm}
% The second case study utilizes a utility-scale BESS with 6 MW rated power and 48 MWh capacity deployed in the grid at one of the feeders. From the technology optimization side, it is assumed that the BESS has been instructed to follow an hourly active power dispatched profile of one day~\cref{fig-RealPower}. It is assumed that this active power injections are fixed for these time steps after being calculated through a pre-defined optimization routine with an assumption of unity power-factor. The proposed algorithm then optimizes reactive power to improve grid conditions, where maximum reactive power of the BESS is 3.6 MVar, given  the inverter size is 7 MVA. For a heavily loaded grid, usually, a higher reactive power draw causes higher losses, so we limit the minimum reactive power capability of BESS at -2.4 MVAr. The penalty of deviating from the preferred schedule is fixed as 2 units/MVar$^2$.
% \begin{figure}[h]
% \centering
% \includegraphics[width=0.4\textwidth]{extras/Figures/reactive_voltage.eps}
% \caption{Before (dashed lines) and after optimization (solid lines) of reactive power (top) and voltages at one of the nodes closer to the BESS (bottom).}
%  \label{fig-Nantucket-Voltages}
% \end{figure}
% From \cref{fig-Nantucket-Voltages}, it can be seen that through reactive power optimization, the voltages are brought back to their minimum/maximum limits. Similar to the case of controllable loads, it can be imagined that not all voltages in the grid are brought within the strict limits of 0.95-1.05 per-unit. Nevertheless, total minimum voltage violation count (for all time steps) comes down from 83,662 to 37,609, whereas the maximum voltage violation count reduces from 46,905 to 44,943.
% \begin{figure}[h]
% \centering
% \includegraphics[width=0.4\textwidth]{extras/Figures/current_losses.eps}
% \caption{Before (dashed lines) and after optimization (solid lines) line currents at one of the major lines in the feeder containing the BESS (top) and losses of the overall grid (bottom).}
%  \label{fig-Nantucket-losses}
% \end{figure}
% \Cref{fig-Nantucket-losses} shows that the proposed method brings line currents within the allowable limits. During BESS discharging hours (14-21), line currents are already within the limits, which is then utilized by the algorithm to draw reactive power and move some of the voltages to avoid maximum voltage violations \cref{fig-Nantucket-Voltages}. The total grid losses for the charging hours reduced from 7.2 MW to 7.0 MW, whereas for the discharging hours, due to reactive power draw, increased from 4.42 MW to 4.45 MW. 
% \vspace{-0.25cm}


==> nomeclature.tex <==
% LIST OF ACRONYMS AND SYMBOLS

% General Terms

%\newglossaryentry{}{type=\acronymtype, name={}, description={}, user1={},sort={}}
\newglossaryentry{adg}{type=\acronymtype, name={ADG}, description={Active Distribution Grids}, user1={},sort={}}
\newglossaryentry{ed}{type=\acronymtype, name={ED}, description={Economic Dispatch}, user1={},sort={}}
\newglossaryentry{fdla}{type=\acronymtype, name={FDLA}, description={fastest distributed linear averaging}, user1={},sort={}}
\newglossaryentry{res}{type=\acronymtype, name={RES}, description={renewable energy sources}, user1={},sort={}}
\newglossaryentry{dg}{type=\acronymtype, name={DG}, description={distributed generators}, user1={},sort={}}
\newglossaryentry{der}{type=\acronymtype, name={DER}, description={distributed energy resources}, user1={},sort={}}
\newglossaryentry{mas}{type=\acronymtype, name={MAS}, description={multi-agent system}, user1={},sort={}}
\newglossaryentry{oltc}{type=\acronymtype, name={OLTC}, description={on load tap changer}, user1={},sort={}}
\newglossaryentry{sc}{type=\acronymtype, name={SC}, description={switched capacitors}, user1={},sort={}}
\newglossaryentry{cnp}{type=\acronymtype, name={CNP}, description={control net protocol}, user1={},sort={}}
\newglossaryentry{mtids}{type=\acronymtype, name={MTIDS}, description={MATLAB Toolbox for Interconnected Dynamical Systems}, user1={},sort={}}
\newglossaryentry{pcc}{type=\acronymtype, name={PCC}, description={point of common coupling}, user1={},sort={}}
\newglossaryentry{cast}{type=\acronymtype, name={CAST}, description={consensus-ADMM structured TR}, user1={},sort={}}
\newglossaryentry{psp}{type=\acronymtype, name={PSP}, description={power supply point}, user1={},sort={}}
\newglossaryentry{acopf}{type=\acronymtype, name={ACOPF}, description={AC optimal power flow}, user1={},sort={}}
\newglossaryentry{opf}{type=\acronymtype, name={OPF}, description={optimal power flow}, user1={},sort={}}
\newglossaryentry{dso}{type=\acronymtype, name={DSO}, description={Distribution System Operator}, user1={},sort={}}
\newglossaryentry{fcvs}{type=\acronymtype, name={FCVS}, description={fast consensus-based voltage support}, user1={},sort={}}
\newglossaryentry{kkt}{type=\acronymtype, name={KKT}, description={Karush-Kuhn-Tucker}, user1={},sort={}}
\newglossaryentry{admm}{type=\acronymtype, name={ADMM}, description={alternating direction method of multipliers },plural={alternating direction method of multipliers}, user1={},sort={}}
\newglossaryentry{dcopf}{type=\acronymtype, name={DC-OPF}, description={DC optimal power flow}, user1={},sort={}}
\newglossaryentry{tr}{type=\acronymtype, name={TR}, description={trust region}, user1={},sort={}}
\newglossaryentry{tso}{type=\acronymtype, name={TSO}, description={transmission system operator}, user1={},sort={}}
\newglossaryentry{sgo}{type=\acronymtype, name={SGO}, description={smart grid operator}, user1={},sort={}}
\newglossaryentry{mgo}{type=\acronymtype, name={MGO}, description={microgrid operator}, user1={},sort={}}
\newglossaryentry{dlmp}{type=\acronymtype, name={DLMP}, description={distribution locational marginal price}, user1={},sort={}}
\newglossaryentry{lmp}{type=\acronymtype, name={LMP}, description={locational marginal pricing}, user1={},sort={}}
% Sets, Indices
\newglossaryentry{graph}{type=set, name={$G$}, description={Communication graph}, user1={},sort={graph}}
\newglossaryentry{Vs}{type=set, name={$V$}, description={Node set of communication graph}, user1={},sort={ns}}
\newglossaryentry{Es}{type=set, name={$E$}, description={Edge set of communication graph}, user1={},sort={es}}
\newglossaryentry{Ni}{type=set, name={$Ni$}, description={Set of neighbor nodes of node $i$ }, user1={},sort={ni}}
\newglossaryentry{k}{type=set, name={$k$}, description={Discrete time index }, user1={},sort={k}}
\newglossaryentry{t}{type=set, name={$t$}, description={Continuous time index }, user1={},sort={t}}

\newglossaryentry{IJ}{type=set, name={$i,j$}, description={Index for DG controller (agent)}, user1={},sort={ij}}
\newglossaryentry{leadJ}{type=set, name={$l$}, description={Index for leading DG controller (agent)}, user1={},sort={lead}}
	
% Param
\newglossaryentry{delPg}{type=parameter, name={$\Delta Q_{i}^{G}$}, description={Active power generation at $i$th bus }, user1={},sort={pg}}
\newglossaryentry{delQg}{type=parameter, name={$\Delta Q_{i}^{G}$}, description={Reactive power generation at $i$th bus}, user1={},sort={Qg}}
\newglossaryentry{delPd}{type=parameter, name={$\Delta P_{i}^{D}$}, description={Active power demand at $i$th bus  }, user1={},sort={Qg}}
\newglossaryentry{delQd}{type=parameter, name={$\Delta Q_{i}^{D}$}, description={Reactive power demand at $i$th bus  }, user1={},sort={Qg}}
\newglossaryentry{cpower}{type=parameter, name={$S_{i}$}, description={Complex power at $i$th bus  }, user1={},sort={cpower}}



\newglossaryentry{delP}{type=parameter, name={$\Delta P$}, description={Active power variation }, user1={},sort={p}}
\newglossaryentry{delQ}{type=parameter, name={$\Delta Q$}, description={Reactive power variation }, user1={},sort={q}}
\newglossaryentry{delV}{type=parameter, name={$\Delta V$}, description={Node voltage variation }, user1={},sort={v}}
\newglossaryentry{delT}{type=parameter, name={$\Delta \theta$}, description={Node angle variation }, user1={},sort={theta}}
\newglossaryentry{sens}{type=parameter, name={$\rho $}, description={Voltage versus reactive power sensitivity coefficient matrix}, user1={},sort={rho}}
\newglossaryentry{sensji}{type=parameter, name={$\rho_{ji} $}, description={Sensitivity coefficient for node voltage at $i$th DG site versus reactive power at $j$th DG site }, user1={},sort={rhoji}}
\newglossaryentry{NoN}{type=parameter, name={$N$}, description={ Number of DG controllers (agents)}, user1={},sort={non}}
\newglossaryentry{acf}{type=parameter, name={$r_{asym}$}, description={Asymptotic convergence factor}, user1={},sort={acf}}
\newglossaryentry{ct}{type=parameter, name={$\tau$}, description={Convergence time}, user1={},sort={ct}}
\newglossaryentry{ss}{type=parameter, name={$\alpha$}, description={Discrete time step size }, user1={},sort={ss}}
\newglossaryentry{phi}{type=parameter, name={$\phi_{i}$}, description={Reactive power constraint for $i$th DG agent }, user1={},sort={phi}}
\newglossaryentry{phi_max}{type=parameter, name={$\phi_{i}^{max}$}, description={Maximal reactive power  dispatch for $i$th DG agent }, user1={},sort={phi_max}}
\newglossaryentry{aij}{type=parameter, name={$a_{ij}$}, description={Adjacency matrix entries of graph $G$}, user1={},sort={aij}}
\newglossaryentry{bij}{type=parameter, name={$b_{ij}$}, description={Modified Laplacian entries}, user1={},sort={bij}}
\newglossaryentry{L}{type=parameter, name={$L$}, description={Graph Laplacian}, user1={},sort={L}}
\newglossaryentry{H}{type=parameter, name={$H$}, description={Perron matrix of graph $G$}, user1={},sort={L}}
\newglossaryentry{A}{type=parameter, name={$A$}, description={Graph adjacency matrix}, user1={},sort={L}}

\newglossaryentry{W}{type=parameter, name={$W$}, description={Modified graph Laplacian}, user1={},sort={W}}
\newglossaryentry{mh}{type=parameter, name={$H_{w}$}, description={Modified Perron matrix of graph $G$}, user1={},sort={mh}}
\newglossaryentry{w}{type=parameter, name={$w_{ji}$}, description={Weighting factor of information from agent $j$ to agent $i$ }, user1={},sort={w}}
\newglossaryentry{beta}{type=parameter, name={$\beta$}, description={Constant edge optimization object}, user1={},sort={beta}}
\newglossaryentry{lambda}{type=parameter, name={$\lambda_{z}$}, description={$z$th biggest eigenvalue of $I-L$}, user1={},sort={lamda}}
\newglossaryentry{ns}{type=parameter, name={$n$}, description={Number of buses in distribution system}, user1={},sort={ms}}
\newglossaryentry{nss}{type=parameter, name={$m$}, description={Number of neighbored buses}, user1={},sort={ms}}
% Variables
\newglossaryentry{x}{type=variable, name={$x_{i}$}, description={Integrator controller state}, user1={},sort={xi}}

\newglossaryentry{Ks}{type=parameter, name={$K$}, description={Integrator gain in constant edge method}, user1={},sort={Ks}}
\newglossaryentry{Qo}{type=variable, name={$\Delta Q^{*}_{i}$}, description={Reactive power variation value for agent $i$ }, user1={},sort={Qo}}
\newglossaryentry{vi}{type=variable, name={$v_{i}^{I}$}, description={$i$th Integrator state of first consensus process}, user1={},sort={vi}}
\newglossaryentry{vii}{type=variable, name={$v_{i}^{II}$}, description={$i$th Integrator state of second consensus process}, user1={},sort={vii}}








